SeMLaPS: Real-time Semantic Mapping with Latent Prior Networks and Quasi-Planar Segmentation

The availability of real-time semantics greatly improves the core geometric functionality of SLAM systems, enabling numerous robotic and AR/VR applications. We present a new methodology for real-time semantic mapping from RGB-D sequences that combines a 2D neural network and a 3D network based on a SLAM system with 3D occupancy mapping. When segmenting a new frame we perform latent feature re-projection from previous frames based on differentiable rendering. Fusing re-projected feature maps from previous frames with current-frame features greatly improves image segmentation quality, compared to a baseline that processes images independently. For 3D map processing, we propose a novel geometric quasi-planar over-segmentation method that groups 3D map elements likely to belong to the same semantic classes, relying on surface normals. We also describe a novel neural network design for lightweight semantic map post-processing. Our system achieves state-of-the-art semantic mapping quality within 2D-3D networks-based systems and matches the performance of 3D convolutional networks on three real indoor datasets, while working in real-time. Moreover, it shows better cross-sensor generalization abilities compared to 3D CNNs, enabling training and inference with different depth sensors. Code and data will be released on project page: http://jingwenwang95.github.io/SeMLaPS

==> Tables/scannet_2d_per_class.tex <==
\begin{table*}
\caption{2D Semantic segmentation on ScanNet v2 (Val)}
\label{tab:scannet2D_per_class}
\begin{center}
\setlength\tabcolsep{1.5pt}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
Method &  mIoU & bath & bed & bkshf & cab & chair & cntr & curt & desk & door & floor & other & pic & fridge & shwr & sink & sofa &tbl & toilet & wall & win\\
\hline
\hline
\multicolumn{22}{|c|}{\bf Single-view inference} \\
\hline
LPN-base & 65.1 & 82.8 & 79.4 & 63.8 & 56.3 & 73.9 & 53.6 & 62.5 & 55.2 & 57.2 & 91.1 & 42.2 & 34.6 & 64.7 & 63.4 & 63.4 & 68.6 & 69.3 & 86.6 & 80.0 & 53.2 \\ 
MVCNet-S~\cite{ma2017multi} & 66.2 & 84.4 & 78.5 & 63.4 & 58.2 & 73.8 & 53.2 & 62.3 & 56.8 & 62.1 & 91.1 & 44.5 & 40.5 & 64.7 & 65.5 & 63.2 & 68.5 & 69.7 & 85.1 & 82.2 & 56.4 \\
LPN-S & 66.5 & 83.2 & 79.2 & 62.8 & 58.7 & 73.0 & 54.8 & 61.9 & 59.1 & 62.1 & 91.1 & 44.9 & 38.5 & 68.0 & 65.7 & 63.0 & 67.3 & 71.3 & 86.0 & 82.2 & 57.8 \\
\hline
\multicolumn{22}{|c|}{\bf Multi-view inference} 
\\
\hline
MVCNet-M3~\cite{ma2017multi} & 68.6 & 86.4 & 80.6 & 65.2 & 60.9 & 76.0 & 55.9 & 66.0 & 60.4 & 65.1 & 91.5 & 47.4 & 41.9 & 68.1 & 67.7 & 65.1 & 71.9 & 72.0 & 87.4 & 83.6 & 58.7 \\
LPN-M3 &  69.0 & 85.7 & 81.3 & 65.0 & 61.3 & 75.3 & 57.4 & 65.5 & 62.5 & 65.4 & 91.4 & 48.1 & 39.9 & 71.5 & 68.5 & 64.7 & 70.7 & 73.4 & 87.6 & 83.4 & 60.7 \\
LPN-M5 &  69.7 & 86.1 & 81.9 & 65.7 & 62.3 & 75.8 & 58.1 & 66.8 & 63.6 & 66.6 & 91.4 & 49.4 & 40.5 & 72.7 & 69.5 & 65.0 & 72.1 & 74.0 & 87.7 & 83.7 & 61.8 \\
LPN-M7 &  70.1 & 86.2 & 82.2 & 66.1 & 62.8 & 76.1 & 58.6 & 67.3 & 64.1 & 67.1 & 91.3 & 50.2 & 40.8 & 73.4 & 69.8 & 65.2 & 72.9 & 74.3 & 87.6 & 83.8 & 62.2 \\
\hline
% \multicolumn{23}{|c|}{\bf Whole sequence inference} 
% \\
% \hline
% BP-Net~\cite{hu2021bidirectional} & - & 67.0& 82.2& 79.5& 83.6& 65.9& 48.1& 45.1& 76.9& 65.6& 56.7& 93.1& 39.5& 39.0& 70.0& 53.4& 68.9& 77.0& 57.4& 86.5& 83.1& 67.5 \\
% \hline
\end{tabular}
\end{center}
\end{table*}

==> Tables/scannet_3d_brief.tex <==
\begin{table*}[ht]
\caption{3D Semantic segmentation on ScanNet v2 (Val). \vspace{-6pt}}
\label{tab:scannet3d}
\begin{center}
\setlength\tabcolsep{1.5pt}
\begin{tabular}{|c|c|c|}
\hline
Method & Type & mIoU\\
\hline
\hline
\multicolumn{3}{|c|}{\bf 3D networks} \\
\hline
% BP-Net~\cite{} & - & - & 74.9& 90.9& 81.8& 81.1& 75.2& 83.9& 48.5& 84.2& 67.3& 64.4& 95.7& 52.8& 30.5& 77.3& 85.9& 78.8& 81.8& 69.3& 91.6& 85.6& 72.3 \\
MkNet~\cite{choy20194d} & offline & 72.2 \\
SparseConvNet~\cite{graham20183d} & offline & 69.3 \\
INS-CONV~\cite{liu2022ins} & online & 71.5  \\
INS-CONV~\cite{liu2022ins} & online & \textbf{72.4}  \\
\hline
\multicolumn{3}{|c|}{\bf 2D-3D networks} \\
\hline
PsF~\cite{pham2019real} & online & 55.0  \\
FPC~\cite{zhang2020fusion} & online & 67.2 \\
SVCNN~\cite{huang2021supervoxel} & online & 68.3  \\
\methodname (ours) & online & \textbf{72.2}  \\
\hline
\end{tabular} \vspace{-1.5em}
\end{center}
\end{table*}

==> Tables/smr_brief.tex <==
\begin{table*}[t]
\caption{Semantic Mapping with RealSense: 3D Semantic segmentation. \vspace{-6pt}}
\label{tab:slamcore}
\begin{center}
\setlength\tabcolsep{1.5pt}
\begin{tabular}{c|c|c}
%\hline
%\multicolumn{18}{c}{Semantic Mapping with RealSense} \\
\hline
Method & mAcc & mIoU \\
\hline
SparseConvNet~\cite{graham20183d} & 71.4 & 26.5 \\
\methodname-RGB & {\bf 75.3} & {\bf 44.7} \\
\hline
\end{tabular}
\end{center}
\vspace{-12pt}
\end{table*}
